$K_{\rm L}\rightarrow\mu^+\mu^-$ from lattice QCD

We propose a lattice-QCD-suitable framework for computing the two-photon long-distance contribution to the complex $K_{\rm L}\rightarrow\mu^+\mu^-$ decay amplitude, where QED is treated perturbatively in the continuum and infinite-volume. We provide preliminary numerical results on the quark-connected diagrams on one ensemble at physical pion mass from this method, with well-controlled systematic errors. The successful application of this method will allow the determination of the dispersive part of the aforementioned contribution from first-principles and enable a meaningful comparison between the Standard-Model prediction and experiment.

==> Figures/KtoMuMu_SD.tex <==
%\begin{minipage}{0.27\textwidth}
\begin{tikzpicture}[scale=1]
  \begin{feynman}
    \node [inner sep=0] (i1) at (0, 1) {$d$};
    \node [inner sep=0] (i2) at (0, -1) {$\overline s$};
    \node [inner sep=0, fill] (a) at (1, 1) {};
    \node [inner sep=0, fill] (b) at (1, -1) {};
    \node [inner sep=0, fill] (c) at (3, 1) {};
    \node [inner sep=0, fill] (d) at (3, -1) {};
    \node [inner sep=0] (f1) at (4, 1) {$\mu^{-}$ };
    \node [inner sep=0] (f2) at (4, -1) {$\mu^{+}$ };
    \diagram*{
      {[edges={fermion}]
        (i1) --  (a) -- (b) -- (i2),
        (f2) --  (d) -- (c) -- (f1),
      },
      {[edges={photon}]
        (a) --[edge label=$W^-$] (c),
        (b) --[edge label=$W^+$] (d)
      },
    };
  \end{feynman}
%\end{tikzpicture}
%\end{minipage}
\hspace{180pt}
%\begin{minipage}{0.27\textwidth}
%\vspace{60pt}
%\begin{tikzpicture}[scale=1]
  \begin{feynman}
    \node [inner sep=0] (i1) at (0, 1) {$d$};
    \node [inner sep=0] (i2) at (0, -1) {$\overline s$};
    \node [inner sep=0, fill] (a) at (1, 1) {};
    \node [inner sep=0, fill] (b) at (1, -1) {};
    \node [inner sep=0, fill] (c) at (2, 0) {};
    \node [inner sep=0, fill] (d) at (3, 0) {};
    \node [inner sep=0] (f1) at (4, 1) {$\mu^{-}$ };
    \node [inner sep=0] (f2) at (4, -1) {$\mu^{+}$ };
    \diagram*{
      {[edges={fermion}]
        (i1) --  (a) -- (b) -- (i2),
        (f2) --  (d) -- (f1),
      },
      {[edges={photon}]
        (a) --[edge label=$W^-$]  (c) --[edge label=$W^+$] (b),
        (c) --[edge label=$Z^0$] (d)
      },
    };
  \end{feynman}
\end{tikzpicture}
%\end{minipage}
%\hspace{-60pt}
%\begin{minipage}{0.3\textwidth}
%\vspace{-50pt}
\\
\hspace{100pt}
\begin{tikzpicture}[scale=1.0]
  \begin{feynman}
    \node [inner sep=0] (i1) at (0, 1) {$d$};
    \node [inner sep=0] (i2) at (0, -1) {$\overline s$};
    \node [inner sep=0, fill] (a) at (1, 1) {};
    \node [inner sep=0, fill] (b) at (1, -1) {};
    \node [inner sep=0, fill] (c) at (2, 1) {};
    \node [inner sep=0, fill] (d) at (2, -1) {};
    \node [inner sep=0, fill] (e) at (4, 1) {};
    \node [inner sep=0, fill] (f) at (4, -1) {};
    \node [inner sep=0] (f1) at (5, 1) {$\mu^{-}$ };
    \node [inner sep=0] (f2) at (5, -1) {$\mu^{+}$ };
    \diagram*{
      {[edges={fermion}]
        (i1) --  (a) -- (c) -- (d) -- (b) -- (i2),
        (f2) --  (f) -- (e) -- (f1),
      },
      {[edges={photon}]
        (a) --[edge label=$W$]  (b),
      },
      {[edges={photon}]
        (c) --[edge label=$\gamma $]  (e),
        (d) --[edge label=$\gamma $]  (f),
      },
    };
  \end{feynman}
\end{tikzpicture}
%\end{minipage}
